SEER-MoE: Sparse Expert Efficiency through Regularization for Mixture-of-Experts

The advancement of deep learning has led to the emergence of Mixture-of-Experts (MoEs) models, known for their dynamic allocation of computational resources based on input. Despite their promise, MoEs face challenges, particularly in terms of memory requirements. To address this, our work introduces SEER-MoE, a novel two-stage framework for reducing both the memory footprint and compute requirements of pre-trained MoE models. The first stage involves pruning the total number of experts using a heavy-hitters counting guidance, while the second stage employs a regularization-based fine-tuning strategy to recover accuracy loss and reduce the number of activated experts during inference. Our empirical studies demonstrate the effectiveness of our method, resulting in a sparse MoEs model optimized for inference efficiency with minimal accuracy trade-offs.

==> ethical.tex <==
Our proposed SEER-MoE framework, designed to reduce the memory footprint and compute requirements of Mixture-of-Experts (MoEs) models, could present certain ethical challenges and societal risks. One concern is the potential for the pruning and fine-tuning process to inadvertently introduce or amplify original biases in the model, especially if the data used for our processes are not representative. This could lead to unfair or discriminatory outcomes in applications where the model is deployed. Since our method provides a solution to obtain powerful efficient LLMs, there is also the risk of misuse of these powerful models for malicious purposes, such as spreading misinformation or conducting surveillance. 

Mitigation Strategies:

To address these risks, several mitigation strategies can be considered. First, it is crucial to ensure that the datasets used for pruning and fine-tuning are diverse and representative. Moreover, robust security measures and ethical guidelines should be established to prevent misuse of the technology. These can help ensure that the technology is developed and used responsibly.
